Efficient System-Enforced Deterministic Parallelism

Deterministic execution offers many benefits for debugging, fault tolerance, and security. Running parallel programs deterministically is usually difficult and costly, however - especially if we desire system-enforced determinism, ensuring precise repeatability of arbitrarily buggy or malicious software. Determinator is a novel operating system that enforces determinism on both multithreaded and multi-process computations. Determinator's kernel provides only single-threaded, "shared-nothing" address spaces interacting via deterministic synchronization. An untrusted user-level runtime uses distributed computing techniques to emulate familiar abstractions such as Unix processes, file systems, and shared memory multithreading. The system runs parallel applications deterministically both on multicore PCs and across nodes in a cluster. Coarse-grained parallel benchmarks perform and scale comparably to - sometimes better than - conventional systems, though determinism is costly for fine-grained parallel applications.

==> bg.tex <==
\section{Background and Motivation}
\label{sec-bg}

This section briefly reviews some of the reasons
deterministic computing environments are useful,
then outlines reasons it is challenging to achieve determinism
when running software on today's systems.

\subsection{Why Determinism is Useful}

Determinism can be useful for at least three general reasons:
(1) it enables post-mortem execution replay and analysis
to trace bugs or security breaches with minimal logging;
(2) it enables one machine to replicate and/or check
another machine's computation precisely;
(3) it can close timing channels
leading to security and privacy vulnerabilities.

\com{
\subsubsection{Post-mortem analysis}

\subsubsection{Fault Tolerance}

\subsubsection{Accountability}

BFT, peer review etc.

\subsubsection{Information Security}

avoid covert channels

\subsubsection{Migration}

transparently across CPU implementations

\subsubsection{Platform Testing}

FDIV bug?
}%com

\paragraph{Post-Mortem Analysis:}

It is easier to develop and maintain software
when bugs are reproducible,
and a deterministic execution environment ensures that
all computations are exactly reproducible
provided that external inputs are logged.
Time-travel debugging~\cite{curtis82bugnet,leblanc87debugging,
	feldman88igor,pan88supporting,king05debugging}
and intrusion analysis techniques~\cite{dunlap02revirt,joshi05detecting}
rely on execution replay,
for example.
While replay is possible in conventional systems
by logging internal nondeterministic events as well as external inputs,
this additional logging incurs performance and storage costs~\cite
	{choi98deterministic,dunlap08execution},
which may render full-time logging of deployed systems impractical.
Unfortunately, if a bug manifests or malware infection occurs ``in the field''
with logging disabled,
the bug or infection may not recur
during subsequent logged executions in the lab---%
especially with malware designed to detect and avoid
virtualized environments~\cite{raffetseder07detecting}.
If the external inputs to a computation are small
compared with the size of the computation itself,
as in many compute-bound scientific or data analysis applications,
a deterministic environment may make ``full-time'' logging practical
where logging of a comparable nondeterministic environment would not be.

% XXX define "computation management" mechanisms

% XXX make point that programming is just easier in deterministic model

\paragraph{Replication and Verification:}

Determinism enables one machine to replicate
a computation running on another machine exactly.
Standard fault tolerance mechanisms~\cite{
	schneider90implementing,bressoud96hypervisor}
and byzantine fault tolerance (BFT)~\cite{castro99practical}
require replicas to execute deterministically in lock-step,
so that correct replicas always have exactly the same state
and yield the same results after a given sequence of inputs.
Computation accountability mechanisms
such as peer review~\cite{haeberlen07peerreview}
require one machine to verify another's computation
by deterministically re-executing it from a stored snapshot
and comparing the resulting states;
even a semantically inconsequential difference
between processors' intermediate results
can lead to a false alarm in such a system.
Current BFT and peer review systems typically work
only for small ``toy'' computations
that are carefully designed to be fully deterministic
as the model requires;
running large legacy applications under BFT or peer review
would require a level of determinism
that current operating systems do not provide.

%XXX process migration, speculative execution (speculative make on V)?

%\paragraph{Timing Attack Prevention:}
\paragraph{Information Security:}

While many organizations see strong economic or practical motivations
to move compute-intensive applications
onto shared clusters or cloud services such as EC2~\cite{amazon-ec2},
sharing can create considerable information security and privacy concerns.
Even if the cloud provider itself is trustworthy
and its virtualization software correctly prevents
clients from directly interfering with each other,
any client's software can mount a variety of timing attacks
on other client processes running on the same or nearby hosts
to steal valuable secrets~\cite{brumley03remote,percival05cache},
provided the attacking process has fine-grained timing capability.
But many compute-bound applications suited to cloud computing
have no inherent need for fine-grained timing:
most data analysis applications merely compute a result
from a well-defined input dataset.
If a provider offered a compute cloud
in which no client has fine-grained timing capability,
the only timing information with which one client could attack another
would be the much coarser and noisier total job completion times
observed from the clients' own hosts.
A provider cannot create such a ``timing channel-free'' compute cloud
merely by disabling client access to hardware clocks and timers,
however:
an attacker's hosted code could use many other sources of nondeterminism
to regain fine-grained timing capability,
such as by spawning a thread that counts iterations of a spin-loop.
Only fully timing-insensitive execution
can guarantee a shared environment free of timing attack channels.

\com{
% Also: Bonneau, Cache-Collision Timing Attacks Against AES, 2006
%	Cache attacks and countermeasures: the case of AES
%	Predicting secret keys via branch prediction 

honeypot detection in malware.
If software running in a virtual environment has access to timing information,
there are generally many ways it can learn about the virtual environment
it us running in via timing signatures~\cite{garfinkel07compatibility},
and malware can and does use techniques such as these
to evade detection in honeytraps~\cite{raffetseder07detecting}.
}%com

\subsection{Why Determinism is Challenging}

Despite the above benefits,
there are also good reasons true determinism
is difficult to achieve in practice.
We classify these reasons into three categories:
external interactions,
parallel processing,
and heterogeneity.

\paragraph{External Interactions:}
Some applications are fundamentally nondeterministic
because they are semantically dependent on or driven by
interaction with the nondeterministic ``real world'':
on-line transaction processing (OLTP) or real-time systems for example.
In such applications, nondeterministic events arriving from the real world
form a primary part of the ``inputs'' to the system,
and these nondeterministic inputs cannot be eliminated
without changing what the system does.
Applications such as these
are outside of Determinator's primary focus
and are probably better implemented on conventional operating systems.
If such an application has compute-intensive {\em subcomponents}
with well-defined inputs and outputs,
however,
such as the frame encoding/decoding component
of a video streaming application,
these subcomponents might run
in a Determinator ``sandbox'' attached to a conventional OS.
%as outlined later in Section~\ref{XXX}.

\paragraph{Parallel Processing:}

The proliferation of multicore hardware is forcing
ever more developers to write parallel software,
but standard multithreaded programming models
rely entirely on the programmer to control the timing-sensitivity
and consequent nondeterminism of parallel execution,
commonly leading to difficult-to-reproduce ``heisenbugs''~\cite
	{lee06problem,lu08learning}.
%
\com{
While techniques to identify and fix heisenbugs
represent another hot research topic,
it would be better yet if heisenbugs did not exist---%
a property that deterministic environments can provide.
Cloud computing further amplifies
both the challenges of providing determinism,
due to the large-scale parallelism and heterogeneity of a cloud,
and the need for the convenience of a deterministic environment.
If it is painful to find and fix a heisenbug that manifests
only once every thousand test runs in a short-lived application
running on one workstation,
consider the difficulty and expense of finding a heisenbug
requiring thousands of test runs of a data analysis application
distributed across thousands of machines.
}%com
%
As mentioned earlier,
parallel synchronization events may be logged and replayed~\cite
	{feldman88igor,choi98deterministic,dunlap08execution},
but logging incurs performance and storage costs,
and must be initiated {\em before} execution:
a heisenbug that manifests ``in the field''
during non-logged execution
may not reappear during subsequent logged attempts.
Many techniques can help find and fix certain types of heisenbugs~\cite
	{engler03racerx,musuvathi08heisenbugs},
but only deterministic execution eliminates their possibility.
Eliminating unnecessary internal sources of nondeterminism
due to parallel processing is the focus of this proposal.

\paragraph{Heterogeneity:}
In cluster or cloud environments
where an application may be distributed or replicated
across heterogeneous machines,
processor implementation variations
introduce further nondeterminism.
Variations in architecture extensions
cause difficulties migrating virtual machines,
for example~\cite{dipetrillo08migrating,armstrong08virtualization}.
Processors can yield differing results
even for instructions common to all implementations:
many x86 instructions such as MUL and DIV
leave condition codes implementation-defined~\cite{intel09},
and implementations may round
transcendental floating-point results differently
because exact rounding is challenging for basic mathematical reasons~\cite
	{schulte93exact,lefevre01worst,hanrot07worst}.
\com{
causes additional nondeterminism.
Implementations of the same architecture,
such as x86 chips from different vendors or generations,
often support different sets of architectural extensions,
and even yield slightly different results for common instructions
such as those that leave some condition flags undefined~\cite{intel09}
or compute transcendental functions~\cite
	{schulte93exact,lefevre01worst,hanrot07worst}.
Architectural variations cause difficulties migrating virtual machines~\cite
	{dipetrillo08migrating,armstrong08virtualization},
}%com
Even if such variations are ``semantically harmless,''
e.g., because undefined condition codes are ignored by correct code
and inexact rounding causes negligible errors in numerical outputs,
such differences still render
bit-for-bit comparisons of state snapshots impossible,
as required by fault tolerance and accountability mechanisms
such as BFT~\cite{castro99practical}
or peer review~\cite{haeberlen07peerreview}.
Malicious code could also leverage such ``harmless'' variations:
if an attacker knows a company's IDS honeyfarm
to be built on Intel processors,
but the company's overall internal network is heterogeneous,
he might design a virus to evade detection
by acting benignly on Intel processors and subverting only AMD hosts.
We do not address determinism across heterogeneous clusters
in this proposal, but may do so in follow-on work.

\xxx{	If/when we expand on this:
	make clear the attack and defense model -
	e.g., an exploit-finder virus attempts to establish a beachhead,
	then downloads commands and further malware dynamically,
	based on information it detects about the host;
	if this information includes CPU type etc.,
	then the honeyfarm owner will see that an attack occurred
	but it may just look like some generic virus attack,
	whereas the malware running on other internal machines
	might download specific, targeted attack code
	designed to avoid the honeyfarm.
}

\com{	old stuff...
%also:	\item	Easier to write and debug software
%		for deterministic environments:
%		more predictable, fewer heisenbugs.
%		(review concurrency bug literature.)

%	...and all these things are even more necessary
%	in large-scale cloud computing contexts
%	where management becomes the biggest problem.

\com{
\subsubsection{Parallelism}

Requires weak coupling, independence

weakly consistent memory models with complex rules
effectively make modern architectures
even {\em less} deterministic.

\subsubsection{Implementation Tradeoffs}

\subsubsection{Mathematical Challenges}
}%com

Providing deterministic execution environments
is becoming ever more difficult in practice, however,
for two reasons,
both related to recent trends in hardware evolution.
First, as the processor industry moves away from the goal of
ratcheting up the performance of a single-threaded CPU
and toward ever wider multi-socket, multi-core, and multi-thread CPU designs,
leveraging parallelism is becoming a basic requirement of mainstream software,
and with parallelism traditionally comes nondeterminism
due to the subtle timing of standard inter-thread communication models.
Second, as distribution of large computations across nodes
becomes ever more crucial in both traditional datacenter
and emerging cloud computing models,
hardware platform heterogeneity is increasingly injecting
another element of nondeterminism into computing systems:
a computation first run and checkpointed on a cluster
consisting of one particular processor model and stepping
may yield different results if replayed on even a slightly different
(e.g., newer) processor model by the same manufacturer.

While we normally try to design application code
so as to avoid the elements of nondeterminism
inherent in the underlying computing platform---%
e.g., by using synchronization mechanisms properly
to prevent results from being timing-dependent,
and by avoiding reliance on undefined or implementation-dependent values
that certain processor instructions may produce---%
we often need computation management mechanisms to function
even in the presence of {\em incorrect} code.
Debugging mechanisms, for instance, should not have to
fail because the bugs manifest themselves unpredictably.
\com{
Similarly, if a cloud computing customer
uses an accountability mechanism such as peer review~\cite{XXX}
to spot-check the computations of one set of nodes by another
(e.g., across hardware provided and managed
by different cloud computing providers),
...
}

Strict determinism is difficult to provide, however,
for two main reasons.
First, most parallel and distributed execution environments
are highly nondeterministic by nature,
because the actual execution sequence depends on the exact timing
of the interactions between processors or cores
and their relative execution speeds,
which in turn depend on innumerable subtle and unpredictable factors.
Second, even in a single-threaded execution environment,
the exact results of a computation may differ
depending on the specific brand, model, and even stepping
of processor on which it is executing.
If a computation first one on one processor
needs to be replayed on another processor
and the processor implementations do not match exactly,
then the respective computations may diverge,
triggering false alarms in fault tolerance mechanisms for example.
In practice, processor implementations for the same architecture
frequently differ in two significant ways:
in the way they round the results of transcendental floating-point operations,
such as {\tt sin} and {\tt exp};
and in the behavior of instructions
whose effects on certain registers or condition codes
are left architecturally undefined,
such as the effect of an x86 {\tt div} instruction on the condition codes.
Cloud computing environments exacerbate
both of these challenges to providing determinism,
because they must be highly parallel
in order to provide the ``horizontal scalability''
that motivates cloud computing in the first place,
and because a cloud computing cluster may be built incrementally
out of machines purchased at different times
and thus containing processors of different generations or steppings,
even if the cloud computing provider guarantees that all processors
will be of the same vendor and model.
\com{XXX easily testable:
	rent a cluster temporarily from amazon and test the steppings.}

\subsection{Why Determinism is Possible---Even in Clouds}

Nevertheless, potential solutions exist to all of these determinism challenges,
and we believe that fully deterministic cloud computing environments
may be practical and efficient enough
at least for some broad and useful class of applications if not all.
This paper briefly explores this problem and solution space,
and lays out one of many possible approaches
to building a deterministic cloud computing environment.
To address the problems of nondeterminism due to parallelism,
we propose moving away from the classic execution model
in which concurrent processes or threads
simultaneously access one shared resource,
such as a common physical memory or file system,
and towards a model in which concurrent processors or threads
execute in temporary, isolated virtual replicas of shared resources,
which are then reconciled at synchronization points
defined deterministically by the computation itself
rather than nondeterministically by the timing of its execution.
To address the problems of nondeterminism due to processor heterogeneity,
we explore mechanisms to ensure deterministic behavior by
(a) using library implementations of transcendental floating-point functions
in place of native processor-dependent implementations,
(b) using automatic code verification and/or rewriting mechanisms
to ensure that application code cannot depend
on architecturally undefined results from any instruction,
and that such undefined results are never revealed
in the environment's virtual execution state
(e.g., when saving its state to run a signal handler).
}%com

\xxx{ get this point in somewhere...
We expect these determinism-enforcing mechanisms
to come at some performance cost,
which has yet to be evaluated thoroughly;
we believe, however, that if the performance cost is moderate,
even only for certain applications
(e.g., ``embarrassingly parallel'' applications
that do not perform too much fine-grained inter-thread communication
and which do not rely too heavily on transcendental floating-point operations),
cloud computing customers are likely to be willing to rent a few more machines
in exchange for the debugging, manageability, fault tolerance,
and accountability features
that strictly deterministic execution can enable.
The application areas we expect to be most suitable
for running efficiently in such a deterministic environment
include large batch computations such as distributed software builds,
parallel rendering/visualization systems, and distributed data analysis.
We are less hopeful that strict determinism will be useful or practical
for other applications such as transactional processing systems,
which must keep up with a high-bandwidth stream of nondeterministic inputs
and is likely to require fine-grained interprocessor synchronization
to provide classic transaction semantics.

The next two sections detail the problems of providing determinism
in the presence of parallelism and heterogeneity, respectively,
and point out approaches we are exploring to solving these problems.
}


==> determ.tex <==
\section{Provider-Enforced Determinism}

While the proposed solution to timing channels is strong and general,
its practicality hinges on two important questions:
can customers readily implement and run large parallel cloud applications
in a strictly deterministic environment,
and can these deterministic compute jobs run efficiently?
We address the first question in this section,
and the second in Sections~\ref{impl} and~\ref{sec-eval}.

\xxx{make sure other benefits of determinism get mentioned}

\section{Sources of Nondeterminism}

Cloud applications often depend on timers or other nondeterministic inputs
for many reasons,
which we divide into {\em internal} and {\em external dependencies}.
Internal dependencies
are sources of nondeterminism
that may affect the application's internal operation
but do not or should not affect the application's externally visible behavior,
whereas external dependencies are those
that the application fundamentally requires to perform its function.

\paragraph{External dependencies:}
Interactive web applications
need ``wall-clock'' timers to implement application-level network protocols,
session timeouts, real-time user interface updates, etc.
Cryptographic algorithms need sources of (ideally ``true'') randomness
with which to seed cryptographic algorithms.

Compute jobs running under provider-enforced determinism
must obtain any external nondeterministic information they depend on
as part of the explicit inputs at the beginning of a given compute job,
since they cannot obtain such inputs during the compute job.
For highly interactive or time-sensitive interactions, for example,
unshared and unrestricted servers in a customer's private timing domain
could handle the time-sensitive direct interactions with remote clients,
but delegate longer compute-bound tasks to the shared timing domain.
The private intermediary servers
could explicitly supply all nondeterministic inputs required
to each compute job,
such as the current time and random number seeds.

Alternatively, the provider's timing firewalls 
could automatically supply
some standard nondeterministic inputs,
such as the current time,
to compute jobs initiated by remote clients.
Similarly, when a job completes and delivers its results,
it could request the timing firewall 
to initiate a follow-up job automatically at some future time.
Thus, the timing firewalls could provide compute jobs
with nondeterministic inputs from ``just outside the border,''
{\em between} compute jobs though not {\em during} them.
If the provider allows job initiation every ten or hundred milliseconds,
then interactive web applications might be implementable
entirely within the shared domain.

\paragraph{Internal dependencies:}
Standard parallel and distributed programming models
are highly nondeterministic because thread and process behavior
can depend on relative execution order.
Much parallel programming research
focuses on controlling this ``incidental nondeterminism,''
which is usually unwanted~\cite{lee06problem,bocchino09parallel}.
Applications also sometimes use timing dependencies intentionally
for internal optimization:
examples are work queues and load balancers,
whose purpose is typically to assign queued tasks
to the next worker thread to come available
or the back-end server least loaded at the moment.

Provider-enforced determinism
would eliminate both desired and undesired sources of internal nondeterminism
from shared compute jobs.
On the positive side, determinism
simplifies guest application replay and debugging~\cite{
	curtis82bugnet,leblanc87debugging,king05debugging,dunlap08execution},
	% also feldman88igor,pan88supporting,king05debugging,dunlap08execution
and facilitates accountability mechanisms that rely on deterministic replay,
such as byzantine fault tolerance~\cite{castro99practical}
and peer review~\cite{haeberlen07peerreview}.
On the negative side, determinism
eliminates the customer's ability
to implement dynamic load-balancing optimizations
within a compute job:
the customer must instead rely on
the cloud provider's virtualization infrastructure
to perform all necessary internal dynamic optimization.
\xxx{explain more?}

\subsection{Deterministic Consistency}

Although eliminating unwanted determinism from parallel computations
is clearly desirable, it is not easy or necessarily cheap.

~\cite{ford10deterministic}



==> future.tex <==
\section{Future Work}
\label{sec-future}

Combine IFC with downloadable kernel extensions
to allow apps to introduce custom dynamic scheduling policies
without violating determinism guarantee.

virtual page promises - address I/O bottleneck in root process,
allow nonhierarchical dependency structures, etc.

Resource management:
Current prototype doesn't do demand paging at all
except for copy-on-write,
but could easily page to disk and/or over the network.


file system persistence:
two approaches - KeyKOS/L3 style full-system, 
or implement in the kernel or root process
and checkpoint changes that propagate up the tree from children.


also naturally prevents TOCTTOU vulnerabilities,
and provides race detection...


